Boosting Latent Diffusion Models via Disentangled Representation Alignment

Latent Diffusion Models (LDMs) rely heavily on the compressed latent space provided by Variational Autoencoders (VAEs) for high-quality image generation. Recent studies have attempted to obtain generation-friendly VAEs by directly adopting alignment strategies from LDM training, leveraging Vision Foundation Models (VFMs) as representation alignment targets. However, such alignment paradigms overlook the fundamental differences in representational requirements between LDMs and VAEs. Simple feature mapping from local patches to high-dimensional semantics can induce semantic collapse, leading to the loss of fine-grained attributes. In this paper, we reveal a key insight: unlike LDMs that benefit from high-level global semantics, a generation-friendly VAE must possess strong semantic disentanglement capabilities to preserve fine-grained, attribute-level information in a structured manner. To address this discrepancy, we propose the Semantic-Disentangled VAE (Send-VAE). Deviating from previous shallow alignment approaches, Send-VAE introduces a non-linear mapping architecture to effectively bridge the local structures of VAEs and the dense semantics of VFMs, thereby encouraging emergent disentangled properties in the latent space without explicit regularization. Extensive experiments establish a new paradigm for evaluating VAE latent spaces via low-level attribute separability and demonstrate that Send-VAE achieves state-of-the-art generation quality (FID of 1.21) on ImageNet 256x256.

==> section/related_work.tex <==
\section{Related work}

\textbf{Tokenizers for Image Generation. }
% Image tokenizer aims at transforming the high-dimension images into more compact and
% structured latent representations for downstream works such as generation and  understanding.
Image tokenizers are designed to transform high-dimension image inputs into more compact and structured latent representations, facilitating modeling by downstream generative models.
These tokenizers can be broadly categorized into continuous and discrete types. Continuous tokenizers, exemplified by Variational Autoencoders (VAEs)~\cite{kingma2013auto}, are widely adopted in diffusion-based generation models~\cite{rombach2022high, peebles2023scalable, ma2024sit}; whereas discrete tokenizers, represented by VQGAN~\cite{esser2021taming}, are commonly used in autoregressive (AR) generation models.
However, as these tokenizers are typically trained with a pixel-level reconstruction objective, their latent spaces may not be well aligned with the requirements of generation tasks. 
% To address this limitation, recent researches begin to incorporate semantic information into the training of image tokenizers, with the goal of learning latent spaces that are more suitable for generation.
To tackle this challenge, recent studies have explored training VAEs by aligning their latent representations with the feature spaces of vision foundation models, drawing inspiration from recent advances in the training of diffusion transformers~\cite{yu2025representation}.
For instance, VA-VAE~\cite{yao2025reconstruction} aligns the latent representations of VAE with pre-trained vision foundation models, significantly improving the generation performance of high-dimensional tokenizers while preserving their original reconstruction capabilities. 
Inspired by MAE~\cite{he2022masked}, MAETok~\cite{chen2025masked} incorporates masked image modeling into tokenizer training and leverages multiple target features to learn a semantically rich latent space. 
Similar strategies have also been explored in discrete tokenizers~\cite{xiong2025gigatok, li2025imagefolder}.
While these strategies deliver appreciable gains, applying an identical alignment target to both VAEs and LDMs neglects their inherently distinct representational requirements. In contrast to explicit alignment-based approaches, REPA-E~\cite{leng2025repa} adopts an end-to-end joint training framework, backpropagating the representation alignment loss from diffusion transformers to the VAE. Although REPA-E achieves notable performance improvements, its straightforward joint training paradigm leaves a fundamental question unresolved: what characteristics make a VAE particularly well-suited for generation tasks?
We posit that the representational needs of LDMs and VAEs differ at a fundamental level, and argue that an effective generation-friendly VAE should exhibit strong semantic disentanglement capabilities. To this end, we harness the semantically rich representations from pre-trained vision foundation models to guide the VAE’s learning process.

